Improved skin lesion recognition by a Self-Supervised Curricular Deep Learning approach

State-of-the-art deep learning approaches for skin lesion recognition often require pretraining on larger and more varied datasets, to overcome the generalization limitations derived from the reduced size of the skin lesion imaging datasets. ImageNet is often used as the pretraining dataset, but its transferring potential is hindered by the domain gap between the source dataset and the target dermatoscopic scenario. In this work, we introduce a novel pretraining approach that sequentially trains a series of Self-Supervised Learning pretext tasks and only requires the unlabeled skin lesion imaging data. We present a simple methodology to establish an ordering that defines a pretext task curriculum. For the multi-class skin lesion classification problem, and ISIC-2019 dataset, we provide experimental evidence showing that: i) a model pretrained by a curriculum of pretext tasks outperforms models pretrained by individual pretext tasks, and ii) a model pretrained by the optimal pretext task curriculum outperforms a model pretrained on ImageNet. We demonstrate that this performance gain is related to the fact that the curriculum of pretext tasks better focuses the attention of the final model on the skin lesion. Beyond performance improvement, this strategy allows for a large reduction in the training time with respect to ImageNet pretraining, which is especially advantageous for network architectures tailored for a specific problem.

==> arXiv - SSL pretext task ordering for improved skin lesion recognition/conclusion.tex <==
\section{Conclusions}
\label{sec:Conclusions}

We explore the use of a sequential self-supervised pretraining pipeline to improve the accuracy of skin lesion classification from dermatoscopic images. We show that a model pretrained using a sequence of self-supervised pretext tasks on the target skin lesion dataset outperform models pretrained with individual pretext tasks, and a model pretrained on the ImageNet dataset in a supervised way. This approach also outperforms other top-performing solutions to the multi-class skin lesion recognition problem on the ISIC-2019 dataset, such as model ensembles. The qualitative analysis of the results shows that this strategy helps to better tune the focus of the model on the relevant parts of the image\textemdash skin lesion and its borders.

The experimental results also show that the order of the pretext tasks in the pretraining stage has a crucial effect on the accuracy on the downstream task, and that effective curriculum orderings in the pretext tasks correlate with increasing downstream accuracies obtained for individual pretext task pretraining. However, results also suggest that the optimal ordering are not solely related to the individual pretext task accuracy, but also the similarity in the representations obtained from different pretext tasks. Further work will explore the use of representation similarity metrics to establish optimal curriculum orderings in an automatic manner.  

Furthermore, our approach presents strong benefits for the computational complexity of the pretraining step, with respect to the ImageNet counterpart. It requires only a fraction of the ImageNet training time for relatively small datasets, such as ISIC-2019. This is  especially relevant for ad-hoc network   architectures for which a pretrained  ImageNet model may be unavailable.




\begin{figure}[t]
  \centering
       \includegraphics[width=0.5\textwidth]{figures/CKA_on_individual_tasks.pdf}
       \caption{Similarities of feature maps learned by pretext tasks per layer. The similarity of feature maps is measured with Central Kernel Alignment (CKA): values of CKA closer to 1 indicate strong similarity of feature maps, while values closer to 0 indicate that they are dissimilar. }
  \label{fig_CKA}
\end{figure}

==> arXiv - SSL pretext task ordering for improved skin lesion recognition/discussion.tex <==
\section{Discussion}
\label{sec:Discussion}



It is common ground that transfer learing from a pretrained model usually leads to faster convergence and better performance than training from scratch on natural images~\cite{bib_higher_faster} or skin lesion images~\cite{bib_ssl_isic_2017}. This hypothesis is also confirmed for the models pretrained with SSL pretext tasks, as shown in Section~\ref{sec:Experiments}.
% \todo[inline]{pcl: well, if its not pretrained, there is no tranfer learning ... rephrase pretrained vs from scratch}

% \todo[inline]{pcl: specify in skin lession class.}
 

% \todo[inline]{pcl: a new result is that ... is weird, try to rephrase. Also, since you are doing a brief recap, is important to remark the improvent of multiple pretxt tasks (which had not been explored for skin) and then consider the ordering issues}
To our knowledge, we are the first studying the impact of the ordering of multiple sequential SSL tasks on overall performance gains: the full curriculum setup outperforms all three individual pretext tasks, while the full anti-curriculum setup sits between the two worst-performing single tasks. Interestingly, the highest performance results are obtained by a combination of just two pretext tasks (ODC and MoCo v2) in a curriculum ordering, instead of all three.

% \todo[inline]{pcl: i tend to agree with JC wrt to the adjectives. They are "flowery" but not very descriptive to clarify what is happening. A clearer way to describe it, IMO: talk about basic representations (i.e. specific features that are useful for a specific pretext task but do not generalize to others) vs richer representations (i.e. are useful for a wider range of tasks). If richer, then basic, harm, as features are moved towards the specific narrow-scope ones. It basic, then richer, good if complimentary. liminting the adjectives, but more clearly saying what we mean by them is beneficial for the understanding. Still, is  complicated to be accurate, as these are only hypothesis}

We hypothesize on the reasons behind the effects of different pretext task orderings in the following way; the fact that a pretext task leads to relatively low accuracy after transfer learning, may indicate that only basic pretext task specific features and representations have been learned. Differently, a pretext task resulting in higher downstream performances may be benefiting from the learning of generic features and representations. For this reason, if one of these last \textit{generically}-trained pretext tasks is followed by a \textit{specifically}-trained pretext task, the representations learned at the first stage may be harmed, as they will be countermanded to adapt for solving the specific pretext objective of the second task, loosing its generalization ability. Otherwise, if two pretext tasks result in generic features, their consecutive training is expected to either maintain or improve their individual performance. This reasoning allows to explain why curriculum (and also mixed curriculum) orderings perform better than anti-curriculum ones. 

A pair of pretext tasks ("Best curriculum" on Figure \ref{fig_accuracies}) outperforms a triplet of pretext tasks ("Full curriculum" on Figure \ref{fig_accuracies}), despite containing the same pretext tasks, ordered in the same way. Explicitly, the use of the previous specific-generic hypothesis comparing the best and full curriculum sequences would imply that the first (ODC) and the last (MoCo v2) tasks produce more effective and generic representations than the second task (Relative Location). Under this hypothesis, the presence of Relative Location might harm the overall performance, as MoCO v2 will not improve on the representations of ODC, but will try to \textit{recover} from the representations of Relative Location. However, Relative Location yields a higher downstream performance than ODC. Our hypothesis is that the training directions of ODC and MoCo v2 features are aligned, i.e, they both follow similar training paths, whereas intermediate Relative Location features in the full curriculum somehow \textit{shift} the feature space. 

In order to test this hypothesis we conduct the following experiment: using the Central Kernel Alignment (CKA) \cite{bib_cka} to measure the similarity of representations at different network layers, we compare features learned by the pairs of individual pretext tasks as shown on Figure \ref{fig_CKA}. In accordance with our hypothesis: ODC and MoCo v2 produce very similar representations (the CKA values are close to one for all layers except the final average pooling layer), while the representations of Relative Location are very dissimilar from those of ODC and MoCo v2. This is also a strong evidence of the multi-path training idea, i.e. the fact that two models reaching similar downstream accuracy (as ODC and Relative Location) are relying on dissimilar representations. 

% \todo[inline]{pcl: since the hypotesis and the CKA results are separated, is not clear what you mean with ... two models reach similar accuracies, they do notnecessarily learn similar representations... you need to at least mention which are the similar-performance tasks that have different representations. Also you can use the basic-rich (or any alternative) that you used in the paragraph before, in the discussion at the end of the paragraph}

% \todo[inline]{pcl: i dont see the link between these two things. The reasoning in the second part is clearer. I understand it as ODC and MOCO having similar representations (MOCO more efficient) and Rel Loc a different one. So the Rel Loc in the middle is shifting the feature distribution a lot, so to speak} 
% \todo[inline, color=green]{pcl: instead of the first part, it may be clearer. Something like. 1: Close accuracies not necessarily come from close representations, 2: present CKA as the comparison method for representations, and fig 7. 3: see in Fig how 7 Rel loc and odc are different, (a CKA comparing Rel loc and ODC would be even better, but probably dont have time for that) 4: see how ODC and MOCO are similar in fig 7. 5: the explanation of how Rel loc in the middle decrease the performance \\ kis: I re-wrote the first part, I think it's more clear now. Do you like it this way?} 



% \todo[inline]{pcl: given the text, there is no need to plot CKA before and after Transfer. what insight are these two experiments giving?. In the text below, which of these two are you referring to? If you include the pre- and post-TL comparison one expects to see some conclusion on how a (dis)similarity between features changes after TL}

%  In accordance with our hypothesis: ODC and MoCo v2 produce very similar representations (the CKA values are close to one for all layers except the final avgeage pooling layer), while the representations of Relative Location are very dissimilar from those of ODC and MoCo v2. This is also a strong evidence of the multi-path training idea, i.e. the fact that two models reaching similar downstream accuracy (as ODC and Relative Location) are relying on dissimilar representations. \kis{until here}
 
%   \todo[inline]{pcl: if you have the individual comparisons, use them in the text. It is clearer than using the triplet reference. Say that the representation of  Rel loc is  dissimilar to ODC, even if ther individual accuracy is similar (this links to the initial statement in the discussion)}
    
    % \todo[inline]{pcl: instead of this conclusion I would go for something that can be grounded in our results, and that motivate the more general conclusion in the last paragraph, e.g.. the CKA similarity results (combined with accuracy results) suggest that representation similarity plays a role in the effectiveness of pretext task ordering, besides  individual accuracy only. For instance, REl Loc - ODC- MOCO achieves the second best performance among all combinations (75\%), indicating a benefit from the concatenation of pretext tasks that produce similar representations.}

This discussion also sheds light on the limitations of our approach: while the full curriculum ordering (where all pretext tasks are used) is better than any anti-curriculum and mixed curriculum orderings using all three tasks, it is not always the best option (which also hints that a simple increase of the number pretext tasks in the pretraining pipeline might not lead to better performance). However, we demonstrate that while it is not necessarily the best option, it shows competitive results and in our experiments outperforms the baselines. In this regard, as a direction for the future work, we suggest to incorporate the CKA analysis (alongside individual pretext tasks accuracy) to take into account the relationships between the learned representations of the individual tasks when establishing the curriculum ordering. 
    % \todo[inline]{pcl: i think this last conclusion is quite important (for us) and a clear way to continue exploring. However, there is a risk the reviewers say: well, then conclude something on how to optimize the ordering, and come back when you have finished :) . But lets see ...}

==> arXiv - SSL pretext task ordering for improved skin lesion recognition/experiments.tex <==
\section{Experiments}
\label{sec:Experiments}
% \subsection{Dataset(s)}





\subsection{Setup}

\setlength{\tabcolsep}{4pt}


\begin{table}[t]
\centering
\caption{Comparison of SSL pretraining approaches on the ISIC-2017 binary classification challenge. Pretext-Invariant Representation Learning (PIRL) \cite{bib_pirl} with image transformations produced by the Jigsaw \cite{bib_jigsaw} and Rotation prediction \cite{bib_rotation} pretext tasks, along with individual Relative Location \cite{bib_relative_location}, ODC\cite{bib_odc} and MoCo v2\cite{bib_moco_v2} pretext tasks are outperformed by a combination of Relative Location, ODC and MoCo v2. ROC AUC stands for the area under the receiver operating characteristic curve, PR AUC stands for the area under the precision-recall curve.}
\label{table_isic_2017}
\begin{tabular}{@{}cccc@{}}
\toprule
Starting point & ROC AUC & PR AUC & Accuracy \\ \midrule
Random initialization & 0.598   & 0.257  & 79.67    \\
ImageNet              & 0.791   & 0.525  & 83.03    \\ \midrule
PIRL (Jigsaw) \cite{bib_ssl_isic_2017}         & 0.664   & 0.32   & 79.8     \\
PIRL (Rotation) \cite{bib_ssl_isic_2017}       & 0.732   & 0.37   & 80.3     \\ \midrule
Relative Location     & 0.663   & 0.33   & 78.5    \\
ODC                   & 0.696   & 0.37   & 80.33    \\
MoCo v2               & 0.731   & 0.4    & 80.16    \\ \midrule
\textbf{RL $\,\to\,$ ODC $\,\to\,$ MoCo v2 (ours)} & \textbf{0.754} & \textbf{0.48} & \textbf{82.3} \\ \bottomrule
\end{tabular}
\end{table}
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[]
% \centering
% \caption{The effects of different SSL pretraining strategies on classification accuracy.}
% \label{table_combinations_no_kd}
% \begin{tabular}{@{}rcccccc@{}}
% \toprule
% \multicolumn{1}{c}{} &
%   1st task &
%   2nd task &
%   3rd task &
%   \begin{tabular}[c]{@{}c@{}}Balanced \\ accuracy, \%\end{tabular} &
%   Change, \% &
%   \begin{tabular}[c]{@{}c@{}}Better\\ than\\ ImageNet\end{tabular} \\ \midrule
% -                    & Rel. loc.   &             &             & 69.52 & -     & No           \\
% (AC)                 & Rel. loc.   & ODC         &             & 70.68 & 1.16  & No           \\
% (MC)                 & Rel. loc.   & ODC         & MoCo v2     & 75.00 & 5.49  & \textbf{Yes} \\
% (C)                  & Rel. loc.   & MoCo v2     &             & 74.10 & 4.58  & \textbf{Yes} \\
% (MC)                 & Rel. loc.   & MoCo v2     & ODC         & 74.38 & 4.86  & \textbf{Yes} \\ \midrule
% -                    & MoCo v2     &             &             & 72.74 & -     & No           \\
% (AC)                 & MoCo v2     & ODC         &             & 72.72 & -0.02 & No           \\
% (MC)                 & MoCo v2     & ODC         & Rel. loc.   & 67.00 & -5.74 & No           \\
% (AC)                 & MoCo v2     & Rel. loc.   &             & 66.72 & -6.02 & No           \\
% (AC)                 & MoCo v2     & Rel. loc.   & ODC         & 69.80 & -2.95 & No           \\ \midrule
% -                    & ODC         &             &             & 63.52 & -     & No           \\
% (C)                  & ODC         & Rel. loc.   &             & 68.23 & 4.71  & No           \\
% (C)                  & ODC         & Rel. loc.   & MoCo v2     & 73.36 & 9.84  & No           \\
% (C)                  & ODC         & MoCo v2     &             & 75.44 & 11.92 & \textbf{Yes} \\
% (MC)                 & ODC         & MoCo v2     & Rel. loc.   & 65.73 & 2.21  & No           \\ \midrule
% \multicolumn{1}{c}{} &
%   \multicolumn{3}{c}{ISIC-2019 challenge winner \cite{bib_isic19_winner}} &
%   \begin{tabular}[c]{@{}c@{}}72.5\\ $\pm$1.7\end{tabular} &
%   - &
%   - \\
% \multicolumn{1}{c}{} & \multicolumn{3}{c}{Supervised ImageNet} & 73.76 & -     & -            \\
% \multicolumn{1}{c}{} & \multicolumn{3}{c}{No pretraining}      & 49.27 & -     & -            \\ \bottomrule
% \multicolumn{7}{p{251pt}}{Classification accuracy on ISIC-2019 of ResNet-50 classifiers pretrained on ISIC-2019 with single pretext tasks or their combinations. The right-most column indicates whether the pretraining strategy led to a higher classification accuracy than supervised pretraining on ImageNet. The left-most column shows whether the combination of pretext task follows the curriculum ordering (C), mixed curriculum ordering (MC) or anti-curriculum ordering (AC). 
% }\\
% \end{tabular}
% \end{table}


% \begin{table}[]
% \centering
% \caption{The effects of different SSL pretraining strategies on classification accuracy.}
% \label{table_combinations_no_kd}
% \begin{tabular}{cccccc}
% \hline
% 1st task &
%   2nd task &
%   3rd task &
%   \begin{tabular}[c]{@{}c@{}}Balanced \\ accuracy\end{tabular} &
%   Change &
%   \begin{tabular}[c]{@{}c@{}}Better\\ than\\ ImageNet\end{tabular} \\ \hline
% Rel. loc.   &             &             & 69.52 & -     & No           \\
% Rel. loc.   & ODC         &             & 70.68 & 1.16  & No           \\
% Rel. loc.   & ODC         & MoCo v2     & 75.00 & 5.49  & \textbf{Yes} \\
% Rel. loc.   & MoCo v2     &             & 74.10 & 4.58  & \textbf{Yes} \\
% Rel. loc.   & MoCo v2     & ODC         & 74.38 & 4.86  & \textbf{Yes} \\ \hline
% MoCo v2     &             &             & 72.74 & -     & No           \\
% MoCo v2     & ODC         &             & 72.72 & -0.02 & No           \\
% MoCo v2     & ODC         & Rel. loc.   & 67.00 & -5.74 & No           \\
% MoCo v2     & Rel. loc.   &             & 66.72 & -6.02 & No           \\
% MoCo v2     & Rel. loc.   & ODC         & 69.80 & -2.95 & No           \\ \hline
% ODC         &             &             & 63.52 & -     & No           \\
% ODC         & Rel. loc.   &             & 68.23 & 4.71  & No           \\
% ODC         & Rel. loc.   & MoCo v2     & 73.36 & 9.84  & No           \\
% ODC         & MoCo v2     &             & 75.44 & 11.92 & \textbf{Yes} \\
% ODC         & MoCo v2     & Rel. loc.   & 65.73 & 2.21  & No           \\ \hline
% % \multicolumn{1}{l}{} &
% %   \multicolumn{1}{l}{} &
% %   \multicolumn{1}{l}{} &
% %   \multicolumn{1}{l}{} &
% %   \multicolumn{1}{l}{} &
% %   \multicolumn{1}{l}{} 
% \multicolumn{3}{c}{ISIC-2019 challenge winner} & 72.5 $\pm$ 1.7 & -     & -            \\
% \multicolumn{3}{c}{Supervised ImageNet} & 73.76 & -     & -            \\
% \multicolumn{3}{c}{No pretraining}      & 49.27 & -     & -            \\ \hline
% \multicolumn{6}{p{251pt}}{Classification accuracy on ISIC-2019 of ResNet-50 classifiers pretrained on ISIC-2019 with single pretext tasks or their combinations. The right-most column indicates whether the pretraining strategy led to a higher classification accuracy than supervised pretraining on ImageNet.}\\
% \end{tabular}
% \end{table}

% \todo[inline]{pcl: the explanation in this section is quite mixed. Maybe this alternative works better. 1 Start from the configurations that are common to all experiments: model, SSL training parameters, and fine-tuning parameters. You can refer to figure 2 for clarification. Describe Single-task tests define the ordering. 3 . Describe mult-tasks tests based on the results of single-task tests. }

% \todo[inline]{pcl: Again, i dont feel that we have clearly, formally, formulated an hypothesis. We dont need to, but we need to formulate this first sentence differently, because it is quite confusing as it is. Alternative: something like, ... we follow the method described in Section 3 to assess the effect of sequential pre-training of multiple pretext tasks on the multi-class classification challenge of the ISIC-2019 dataset.}


We follow the method described in Section \ref{sec:Methodology} to assess the effects of sequential pretraining of multiple pretext tasks on the ISIC-2019 multi-class classification challenge (as the latest version of ISIC that addresses the multi-class problem). As consecutive learning of pretext tasks changes the learned representations, it can be expected that same-category pretext tasks learned consecutively will not change the learned representations significantly as they are optimized on the basis of similar objectives (i.e., the representations learned by the pretext tasks of the same category\textemdash \textbf{geometric}, \textbf{clustering} or \textbf{contrastive}\textemdash could be expected to be similar). Therefore, we pick three representative examples of each group of pretext tasks (Relative Location, MoCo v2, ODC) to ensure that the representations learned by them differ between each other, define curriculum orderings and compare them against all other possible combinations of them in the training pipeline. The following steps are used to define the order of pretext tasks:

% \todo[inline]{pcl: See my commenin section 3 about moving a part here. After that part. Say that the next steps are used to define the order}


\begin{enumerate}
    \item Given three pretext tasks, we perform single-source transfer learning with the same target and source domains and record the achieved accuracies: $\mathcal{A}_{RL}, \mathcal{A}_{ODC}, \mathcal{A}_{MoCo\_v2}$. All three pretext tasks use the same backbone architecture: ResNet-50\cite{bib_resnet}.
    
    % \todo[inline]{pcl: reformulate the wording of first step, it seems that you are giving two different substeps, which are in fact the same thing. Also say that the model is the same in the three individual tests}

    \item Following the hypothesis outlined in Section \ref{sec:Methodology} we define as curriculum orderings those coinciding with the increasing single-source transfer learning accuracies (accuracy hereafter). We group all orderings as follows:
    % \item The following pretext task orderings are defined, given the single-source transfer learning accuracies: 
    \begin{itemize}
        \item Curriculum: ordered by increasing accuracy.
        \item Anti-curriculum: ordered by decreasing accuracy.
        \item Full (anti-)curriculum: (anti-)curriculum comprised by all tasks.
    
    \end{itemize}
 Any other ordering is considered a Mixed-curriculum.

    
\end{enumerate}

% \todo[inline]{pcl: i prefer to keep the third point out of the list. Is not really a step for defining orderings,}

% \todo[inline]{pcl: the ...  observe the changes in classification accuracy after transfer learning. ... part is not very informative}
% \todo[inline]{pcl:for the third point refer to the multi-source term that you use after. Section 4B}


Given the individual accuracies of pretext tasks, we define all the curriculum orderings of two and three pretext tasks for the multi-source transfer learning and train corresponding models. Further, in Section \ref{results_main}, we show that these curriculum orderings are the best performing ones (see Tables \ref{table_combinations_no_kd} and \ref{table_isic_2017}), thereby, proving our hypothesis.
% We complement the results with multi-source transfer learning for the combinations of pretext tasks that follow mixed- or anti-curriculum ordering (see Section \ref{results_main}).


Training regimes and hyperparameters for the pretext tasks are presented in Table \ref{table_ssl_params}% and replicate those used in the \href{https://github.com/open-mmlab/OpenSelfSup/blob/master/docs/MODEL_ZOO.md}{OpenSelfSupervised Framework}%
. When transferring the knowledge to the target task, we select the checkpoint from the last pretext task in the pretraining pipeline at the epoch at which the best accuracy is achieved on the validation set (Relative Location) or we simply load the weights from the last epoch when validation set is not available due to the nature of the pretext task (ODC, MoCo v2).

% \todo[inline]{pcl: I moved the baselines after our proposal}

As baselines for comparison we use a model trained from scratch on the target\textemdash skin-lesion recognition\textemdash task (No pretraining) and a model fine-tuned end-to-end on the target task but pre-trained on the ImageNet dataset (Supervised ImageNet). Training hyperparameters for these two models are compiled in the last two rows of Table \ref{table_ssl_params}
% \todo[inline]{pcl: the term Classifier is not used in Table I. In fact, I prefer the one in the table, (no pretraining, more specific)}

% \todo[inline]{pcl: i dont particularly like the term classification task, you can define the target task as the skin-lession recognition task, and use target task hereafter, or use skin-lession recognition. There are many classification tasks involved in the process}

% \todo[inline]{pcl: you are not mentioning here the Resnet-50 model!}


% \todo[inline, color=green]{pcl: I understand that ODC and MOCO do not have a validation set. Then, why not saying that we select the best accuracy on the training set?
% kis: moco also doesn't have an accuracy metric, it just has a loss value and ODC measures training accuracy on the cluster labels that are updated (potentially) at each epoch.}

\subsection{Results for skin-lesion classification} \label{results_main}



\begin{figure}[t]
  \centering
       \includegraphics[width=0.5\textwidth]{figures/Accuracies.pdf}
       \caption{Validation accuracies of classifiers (ResNet-50 models) trained on the features learned with different pretext tasks (or their combinations).}
  \label{fig_accuracies}
\end{figure}
% \todo[inline]{pcl: consider changing this title: Accuracy results for skin-lesion classification?}

% \todo[inline]{pcl: adapt the naming to the one defined in methodology: single-source, multi-source ...}

Table \ref{table_combinations_no_kd} presents the classification accuracies on the ISIC-2019 dataset achieved with different single-source and multi-source transfer learning setups. Given the classification accuracies obtained with the three single-source setups (first row of each block in Table~\ref{table_combinations_no_kd}): $\mathcal{A}_{ODC}=63.5$, $\mathcal{A}_{RL}=69.5$,  $\mathcal{A}_{MoCo\_v2}=72.7$, we define the full curriculum in the multi-source approach as ODC $\,\to\,$ Relative Location  $\,\to\,$ MoCo v2 and the full anti-curriculum as MoCo v2 $\,\to\,$ Relative Location $\,\to\,$ ODC. 

% \todo[inline]{pcl: this bit (below) could go after individual accuracies. Or after multi-source analysis, but here is kinfd of in the middle of nowhere}
% Notably, pretraining only with MoCo v2 already yields results that are competitive with the large ensemble of CNNs that won ISIC-2019 challenge \cite{bib_isic19_winner}.
% \todo[inline]{pcl: Im not sure if it is worth to separate the single task results in a different table, or keep everything in one. If kept in the same, specify where to look for these results, e.g. first row of each block}


% \subsection{Multiple pretext tasks pretraining}

% \todo[inline]{pcl: If we define these categories, urrriculum, mixed curriculum, anticurriculum, I think is worth adding them to the table, for better identification, e.g. C, MC, AC, and expand the acronyms in the caption.  \\kis: Yes, I agree}

The results shown in Table \ref{table_combinations_no_kd} also demonstrate the effect of multi-source pretext task pretraining on the  classification accuracies on ISIC-2019. Specifically, when the pretraining begins with Relative Location or ODC, thereby avoiding the supposed anti-curriculum ordering, the resulting accuracy is always superior to single-source pretext task pretraining. 
% \todo[inline]{pcl:  "classification accuracy obtained after transfer learning" can be simplified }
On the contrary, orderings that are expected to be anti-curriculum (or mixed curriculum) starting with MoCo v2 (e.g., MoCo~v2 $\,\to\,$ ODC; MoCo~v2 $\,\to\,$ ODC $\,\to\,$ RL; MoCo~v2 $\,\to\,$ RL; MoCo~v2 $\,\to\,$ RL $\,\to\,$ ODC) always harm the performance of the individual model (MoCo~v2).
% \todo[inline]{pcl: still not clear which are the references in each comparison. I mean , for us yes, not for a new reader. }

% \todo[inline]{pcl: we have to clarify the ordering in results here....}
% \todo[inline]{pcl: First of all, there must be a paragraph explaining the conditions of the three references that you include in the table, because they are not described by the list of experiments in the experimental setup. So indicating how you obtain them. Specifically, for the ImageNet and No pretrainning you have to clarify the conditions for the target task training, which, are the same described in the Setup?}
% \todo[inline]{pcl: Second, I would avoid the reference to SOTA results, because, Imagenet is already above [3], so it is not clear which is your reference. Use explicit references to [3] or Imagenet-pretrained, and, at the end, we can indicate that to the best of our knowledge, option XX establishes a new SOTA on the problem }
% \todo[inline, color=green]{pcl: question: where does the +-1.7 come from? why they/us dont report the best-case?

% kis: because the validation set isn't public on ISIC-2019, they (and us, and everyone) make their own train/val splits. They repeat it 5 times with different random seeds, so they have 5 different results that are reported as $x\pm y$. 

% mev: In the Table, why the only one with confidence margins is the challenge winner? Why the rest of the models do not have margins associated, how many trials have been performed, only 1?

% kis: yes, we only have one trial per setup
% }

Moreover, five pretraining setups lead to state-of-the-art results after transfer learning, including one where only a single SSL model was trained (MoCo v2); two pretraining setups outperform the current ISIC-2019 winner\cite{bib_isic19_winner} (Relative Location $\,\to\,$ ODC $\,\to\,$ MoCo v2 and ODC $\,\to\,$ MoCo v2); and four pretraining setups outperform the results achieved with fully supervised ImageNet pretraining, with the best result of 75.44\% achieved with a pretraining pipeline of two pretext tasks following a curriculum ordering (ODC $\,\to\,$ MoCo~v2). Overall, combinations of pretext tasks following a curriculum ordering outperform the individual models in all cases and reach the highest performances. Hence, the results support our definition of curriculum.

Figure \ref{fig_accuracies} also demonstrates the accuracy curves on the target task for models pretrained with different setups and reveals that more accurate models do not only reach higher performances but also do it faster than less accurate ones.

To our knowledge, no work targeting a multi-class problem on ISIC-2019 dataset used SSL methods. Therefore, we additionally evaluate our approach on an older version of the ISIC dataset\textemdash ISIC-2017 \cite{bib_isic2017_dataset}\textemdash where SSL approaches were tested before. Table \ref{table_isic_2017} summarizes the results and demonstrates that while none of the three SSL models tested by us (Relative Location, ODC and MoCo v2) outperforms previously published results, their curriculum combination does.

Finally, the bar chart shown on Figure~\ref{fig_bars} indicates that the accuracy gains achieved by different pretraining setups are evenly distributed among all categories of ISIC-2019 and do not come from a large increase in accuracy in only one or few categories:  combinations following the curriculum ordering (ODC $\,\to\,$ MoCo~v2 and ODC $\,\to\,$ RL $\,\to\,$ MoCo~v2) consistently improve the results of the two individual pretext tasks (ODC and MoCo~v2).
% \todo[inline]{pcl: not all bars correspond to improving settings, in fact, some are references. Indicate more where to look in the bars to assess this improvement along all categories}


% \todo[inline]{pcl: we can argue from the results that a general strategy would be to follow the curriculum  order, with something like "step-checking" to see if earli-stopping gives a better configuration (the best accuracy is given by ODC + MOCO. No, not really, early stopping would be odc + rel location. CAn we extract some rules, then?}







\subsection{Qualitative analysis of the results}
\begin{figure}[t]
  \centering
       \includegraphics[width=0.49\textwidth]{figures/bars/all_in_one.pdf}
  
  \caption{Percentage of correctly classified images per class by models with different pretraining strategies.}
  
  \label{fig_bars}
\end{figure}

\begin{figure*}[t]
  \centering
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/no ssl/102_gt.jpg}
    %   \caption{Original}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/no ssl/102_no_ssl.jpg}
       \label{fig_no_ssl_no_ssl}
  \end{subfigure} 
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/no ssl/102_imagenet.jpg}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/no ssl/102_moco.jpg}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/no ssl/102_odc_then_moco.jpg}
  \end{subfigure} 
  \hfill
  \\
  \vspace{-12pt}
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/no ssl/999_gt.jpg}
       \caption{Original}
       \label{fig_no_ssl_a}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/no ssl/999_no_ssl.jpg}
       \caption{No pretraining}
       \label{fig_no_ssl_b}
  \end{subfigure} 
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/no ssl/999_imagenet.jpg}
       \caption{Supervised pretraining (ImageNet)}
       \label{fig_no_ssl_c}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/no ssl/999_moco.jpg}
       \caption{MoCo v2 (best single)}
       \label{fig_no_ssl_d}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/no ssl/999_odc_then_moco.jpg}
       \caption{ODC $\,\to\,$ MoCo v2 (best combination)}
       \label{fig_no_ssl_e}
  \end{subfigure} 
  \caption{Class activation maps of classifiers with and without pretraining on pretext tasks. In the shown samples, classifiers that had no pretraining tend to focus on irrelevant parts of the images (black surrounding areas) and incorrectly classify skin lesions.}
  \label{fig_no_ssl}
\end{figure*}

\begin{figure*}[t]
  \centering
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/moco and odc/198_gt.jpg}
    %   \caption{Original}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/moco and odc/198_odc.jpg}
    %   \caption{ODC}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/moco and odc/198_moco.jpg}
    %   \caption{MoCo v2}
  \end{subfigure} 
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/moco and odc/198_moco_then_odc.jpg}
    %   \caption{MoCo v2 $\,\to\,$ ODC (anti-curriculum)}
  \end{subfigure} 
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/moco and odc/198_odc_then_moco.jpg}
    %   \caption{ODC $\,\to\,$ MoCo v2 (curriculum)}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/moco and odc/79_gt.jpg}
       \caption{Original}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/moco and odc/79_odc.jpg}
       \caption{ODC}
  \end{subfigure} 
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/moco and odc/79_moco.jpg}
       \caption{MoCo v2}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/moco and odc/79_moco_then_odc.jpg}
       \caption{MoCo v2 $\,\to\,$ ODC (anti-curriculum)}
  \end{subfigure} 
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/moco and odc/79_odc_then_moco.jpg}
       \caption{ODC $\,\to\,$ MoCo v2 (curriculum)}
  \end{subfigure}
  \caption{Class activation maps of classifiers pre-trained with ODC and/or MoCo v2. In the presented samples only the curriculum combination of pretext tasks correctly recognizes type of the lesion.
}
  \label{fig_single_tasks_vs_comb_odc_moco}
\end{figure*}




\begin{figure*}[t]
  \centering
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/rl_moco/11_gt.jpg}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/rl_moco/11_relative_location.jpg}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/rl_moco/11_moco.jpg}
  \end{subfigure} 
  ~
  \begin{subfigure}[t]{0.17\textwidth}
    \includegraphics[width=\textwidth]{figures/rl_moco/11_moco_then_relative_locaiton.jpg}
  \end{subfigure} 
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/rl_moco/11_relative_locatino_then_moco.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/rl_moco/31_gt.jpg}
       \caption{Original}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/rl_moco/31_relative_location.jpg}
       \caption{RL}
  \end{subfigure} 
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/rl_moco/31_moco.jpg}
       \caption{MoCo v2}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/rl_moco/31_moco_then_relative_location.jpg}
       \caption{MoCo v2 $\,\to\,$~RL (anti-curriculum)}
  \end{subfigure} 
  ~
  \begin{subfigure}[t]{0.17\textwidth}
       \includegraphics[width=\textwidth]{figures/rl_moco/31_relative_location_then_moco.jpg}
       \caption{RL $\,\to\,$ MoCo v2 (curriculum)}
  \end{subfigure}
  \caption{Class activation maps of classifiers pre-trained with Relative Location and/or MoCo v2. In the presented samples only the curriculum combination of pretext tasks correctly recognizes type of the lesion. RL stands for Relative Location.}
  \label{fig_single_tasks_vs_comb_rl_moco}
\end{figure*}





%In this subsection, using Class Activation Mapping (CAM)\cite{bib_cam} we demonstrate the advantages of using in a pretraining pipeline for transfer learning curriculum orderings of multiple pretext tasks over anti-curriculum orderings and single pretext tasks. Moreover, we visually compare performance of SSL-pretrained models and a model trained from scratch. 
% \todo[inline]{pcl: I've modified this first paragraph. The details of the alternatives are given in the description of figures. NO need to add them here}
Here, we use Class Activation Mapping (CAM)\cite{bib_cam} to demonstrate the advantages of a curriculum ordering of pretext tasks in terms of how accurately the model focuses on areas of the input image that are relevant to the target task. The use of CAM allows to visualizr the discriminative image areas that have a higher impact in the class prediction of a trained network.   
%of multiple pretext tasks over anti-curriculum orderings and single pretext tasks. Moreover, we visually compare performance of SSL-pretrained models and a model trained from scratch. 



% \todo[inline]{pcl: Before going into the conclusions that you can extract from a Figure, you have to give an overview of it. For example, for Figs 3/4 indicate that they contain CAMs for single-task and two-task cases, C and AC, to show the differenes on network-focus in this cases , and justify the selection of ODC-MOCO in one and RELLOC-MOCO in the other}

% \todo[inline]{pcl: After that explanation you can put the consideration of what we think is a good focus. When I mention not to put the conclusions first, I meant  not put first that curriculum focus better, but, to analyze the results you have to put upfront what you consider to be a good focus, i.e. how to interpret the images}

% \todo[inline]{pcl: You have to include somewhere, text or captions, the information on how to interpret the color-grade of the CAMs}

% \todo[inline]{pcl: Also, give more specific guiding of how to interpret the images, like for example AC vs C, how the area of the skin lesion is dark on Fig 3(d) and bright in Fig. 3 (e). Dont just assume the reader is able to interpret the images, or any Figure without any guiding }

% \todo[inline]{pcl: I think that Figure 5 (and its analysis) should go fist. It indicates a higher-level comparison between very different schemes. Then Figures 3-4 shows a finer analysis}


Figure \ref{fig_no_ssl} compares CAMs of models without pretraining, with those using supervised ImageNet or SSL pretraining, Figures \ref{fig_single_tasks_vs_comb_odc_moco} and  \ref{fig_single_tasks_vs_comb_rl_moco} present CAMs of models pretrained with two individual pretext tasks and their combinations arranged according to curriculum or anti-curriculum orderings: Figure \ref{fig_single_tasks_vs_comb_odc_moco} compares the effects of ODC and MoCo v2, and Figure \ref{fig_single_tasks_vs_comb_rl_moco}\textemdash Relative Location and MoCo v2 (we compare ODC and Relative Location against MoCo v2 as it results in the best individual performance).
Figure~\ref{fig_triplets} extends the analysis to the full curriculum and anti-curriculum orderings of pretext tasks.

% \todo[inline]{pcl: You put the analysis of Fig 7 first. So put first, Fig 7 and its description in the paragraph above. This ordering makes sense,as Fig 7 indicates a higher-level comparison between very different schemes.}


% \todo[inline]{pcl: This bit ... (brighter colors mean a higher contribution) ... was included when you were giving a high-level desccription of CAM, which does not make a lot of sense. Integrate it here, where you describe the details of the figures }


Hereinafter, our visual analysis is based on the simple assumption that\textemdash for lesion assessment, the lesion and its borders are more important than other skin tissues (i.e. image regions that are not part of the lesion and its borders).



Figure \ref{fig_no_ssl} presents evidence that for the same input sample image, a non-pretrained model (Figure~\ref{fig_no_ssl_b}) does not focus attention on the skin lesion as much as the pretrained models do (Figures~\ref{fig_no_ssl_c}-\ref{fig_no_ssl_e})\textemdash CAM highlights indicate that a non-pretrained model focuses more attention on the parts of the images that do not contain lesions and gives more importance to the black areas surrounding the image that carry no useful information for image classification. Moreover, Figure \ref{fig_no_ssl_e} demonstrates that the best combination of pretext tasks leads to a model that focuses on the lesions better than the ImageNet-pretrained model: CAM highlights cover the lesion and are absent in other areas of the images (in the presented examples, only the SSL-pretrained models led to the correct classification of skin lesions). Figures~\ref{fig_single_tasks_vs_comb_odc_moco} and \ref{fig_single_tasks_vs_comb_rl_moco} further compare different SSL pretraining setups and show that curriculum ordering of pretext tasks significantly better focuses on the skin lesions than anti-curriculum ordering and individual tasks\textemdash in the CAM images the lesions are highlighted in brighter colors while the rest of the image is dark. In examples presented on Figures \ref{fig_single_tasks_vs_comb_odc_moco}~and~\ref{fig_single_tasks_vs_comb_rl_moco} only the curriculum ordering resulted in the correct classification of skin lesions.

% \todo[inline]{pcl: the discussion of how some mehtodos give relevance to the black areas, has been removed, and I think is important to include it. Instead the information of which samples are classified correctly for each method can go in the caption of the figures, I think} 




% Furthermore, we point out a difference in activation maps produced by models with and without SSL pretraining. A common feature of ISIC-2019 images is black borders around the image caused by the specifics of dermatoscopes. Because these borders have no meaningful information for the skin lesion diagnostics, models that focus attention on these areas should be considered suboptimal. Figure \ref{fig_no_ssl} demonstrates two of many examples when a model that was not pretrained with pretext tasks focuses attention on the aforementioned areas of an image. On the contrary, models pretrained with the single best performing SSL pretext task or the best combination of pretext tasks (according to the classification accuracy from Table \ref{table_combinations_no_kd}) focus more on the lesion itself\textemdash a \textit{behavior} similar to that obtained with supervised pretraining on ImageNet. This shows visual and easily interpretable evidence of superiority of SSL pretraining over the models that had no pretraining. 

% \todo[inline]{pcl: Figure 5 need to be referenced (and described) before the discussion below. Also, be careful with the assumption of SSL-pretraining not focusing on black areas, single mocov2 and odc do focus there in the second example of fig 3. Also, The discussion of Fig 5 focus just exclusively on the black areas. Before that, try to include a general discussion of how the different methods you show in the Fig behave}


% It is, however, important to mention that not all SSL pretraining setups consistently avoid the black areas (Figure \ref{fig_single_tasks_vs_comb_odc_moco} demonstrates a clear example of it). Nevertheless, one can observe that, even in this example where both pretext tasks fail to focus on the lession,  SSL pretraining yields more meaningful CAMs than the "No SSL" setup.



% \todo[inline]{pcl: go upfront in the text of this section with what you want to show with the examples: 1 the contribution of multi-ssl wrt single task (fig 3,4) and whatever you want to show in the configuration of fig 5 :) }


% \todo[inline]{pcl: if you do the whole-page figure, you can probably add all cases of fig 3/4 and 1 in the same figure. Now, maybe the difficulty is to find samples that are good for the 2-task and and 3-task at the same time}

% \subsection{\kis{Verification of visual analysis}}

% \todo[inline]{pcl: I dont see how these graphs are more related to the visual assessment than to the section of accuracy results. In fact I would even add this to the accuracy section, showing that the improvement is consistent along all classes. Also, as it is, the discussion of the graphs does not provide additional information to the conclusions you can extract from the accuracy results. If you add these graphs, they must show something else, which can be the that improvement occurs for all classes, the imbalance, and, something else I am not considering?}

% To support our subjective visual analysis of activation maps, we compare per-class accuracies of models pretrained with different setups. The bar chart shown on Figure \ref{fig_bar_1} indicates that the curriculum ordering of pretext tasks leads to better performing after transfer learning than pretraining solely with either pretext task or their anti-curriculum combination. Similarly, Figure \ref{fig_bar_2} shows that the curriculum ordering of pretext tasks (ODC $\,\to\,$ Relative Location $\,\to\,$ MoCo v2) consistently yields results superior to those achieved with anti-curriculum ordering.

















% \begin{table}[]
% \centering
% \caption{Balanced accuracy of classifiers trained on the features learned by combinations of different SSL models.}
% \label{table_combinations}
% \begin{tabular}{@{}ccccc@{}}
% \toprule
% 1st task &
%   2nd task &
%   3rd task &
%   \begin{tabular}[c]{@{}c@{}}Balanced \\ accuracy\end{tabular} &
%   Change \\ \midrule
% \begin{tabular}[c]{@{}c@{}}Relative Location\\ (scratch no KD)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}MoCo v2 \\ (no KD)\end{tabular} &
%   &
%   74.101 &
%   4.6 \\
% \begin{tabular}[c]{@{}c@{}}Relative Location\\ (ImageNet no KD)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}MoCo v2 \\ (no KD)\end{tabular} &
%   &
%   \textbf{76.921} &
%   11.9 \\
% \begin{tabular}[c]{@{}c@{}}Relative Location\\ (ImageNet KD)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}MoCo v2\\ (no KD)\end{tabular} &
%   &
%   71.937 &
%   5.03 \\
%  &
%   &
%   &
%   &
%   \\
% \begin{tabular}[c]{@{}c@{}}MoCo v2 \\ (scratch no KD)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Relative \\ Location\\ (no KD)\end{tabular} &
%   &
%   66.721 &
%   -6 \\
% \begin{tabular}[c]{@{}c@{}}MoCo v2 \\ (ImageNet no KD)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}ODC \\ (no KD)\end{tabular} &
%   &
%   \textbf{74.742} &
%   -3.3 \\
% \begin{tabular}[c]{@{}c@{}}MoCo v2 \\ (ImageNet no KD)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Relative \\ Location\\ (no KD)\end{tabular} &
%   &
%   65.346 &
%   -12.7 \\
% \begin{tabular}[c]{@{}c@{}}MoCo v2 \\ (ImageNet no KD)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}ODC \\ (no KD)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Relative \\ Location\\ (no KD)\end{tabular} &
%   66.659 &
%   -11.4 \\
%  &
%   &
%   &
%   &
%   \\
% \begin{tabular}[c]{@{}c@{}}ODC \\ (ImageNet no KD)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}MoCo v2 \\ (no KD)\end{tabular} &
%   &
%   \textbf{75.592} &
%   -4.13 \\
% \begin{tabular}[c]{@{}c@{}}ODC \\ (scratch no KD)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}MoCo v2 \\ (no KD)\end{tabular} &
%   &
%   75.442 &
%   11.9 \\
% \begin{tabular}[c]{@{}c@{}}ODC \\ (ImageNet no KD)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Relative \\ Location\\ (no KD)\end{tabular} &
%   &
%   74.576 &
%   -5.2 \\
% \begin{tabular}[c]{@{}c@{}}ODC \\ (scratch no KD)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Relative \\ Location\\ (no KD)\end{tabular} &
%   \multicolumn{1}{l}{} &
%   68.228 &
%   4.7 \\ \bottomrule
% \multicolumn{5}{p{251pt}}{\textcolor{red}{TABLE IN PROGRESS}}\\
% \end{tabular}
% \end{table}

\subsection{Computational complexity of multiple pretext task pretraining}

\setlength{\tabcolsep}{2pt}
\begin{table}
\centering
\caption{Hyperparameters used in the training of SSL and supervised models.}
\label{table_ssl_params}
\begin{tabular}{@{}ccccc@{}}
\toprule
 &
  \begin{tabular}[c]{@{}c@{}}Training\\ epochs\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Batch\\ size\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Learning\\ rate (LR)\end{tabular} &
  LR policy \\ \midrule
Relative location                                              & 70  & 64  & 0.2 & step {[}30; 50{]}                                          \\
MoCo v2                                                        & 200 & 32  & 0.03   & \begin{tabular}[c]{@{}c@{}}Cosine\\ Annealing\end{tabular} \\
ODC                                                            & 200 & 100 & 0.06   & step {[}170{]}                                             \\ \midrule
\begin{tabular}[c]{@{}c@{}}ImageNet\\ pretraining\end{tabular} & 90  & 256 & 0.1    & step {[}30; 60; 90{]}                                      \\
Classifier &
  90 &
  100 &
  0.1 &
  \begin{tabular}[c]{@{}c@{}}step {[}30; 60; 80{]},\\ warm-up: 10 epochs\\ warm-up ratio: 0.0001\end{tabular} \\
  \bottomrule
  \multicolumn{5}{p{251pt}}{The first three rows of the table present the hyperparameters used during pretraining by the SSL models. The last two rows show the hyperparameters used during the ImageNet-pretraining and the hyperparameters used during transferring to the target task.}
\end{tabular}
\end{table}

In this subsection we demonstrate that our proposed SSL-pretraining approach is computationally efficient and requires much less computational effort than typical supervised pretraining on ImageNet. We compare the computational complexity of different pretraining setups by comparing the number of iterations each setup requires to achieve the results indicated in Table~\ref{table_combinations_no_kd}, assuming that the impact on complexity associated with the differences in model architecture for different tasks (SSL or ImageNet-supervised heads) is negligible.

% A fair question that might arise from the analysis of Table \ref{table_combinations_no_kd} is whether pretraining on pretext tasks is more computationally expensive than supervised pretraining on ImageNet.
% We compare the time complexities of different pretraining setups, 
% considering the differences in the number of trainable parameters caused by the differences in the architectures of SSL and supervised classification heads:
% \begin{itemize}
%     \item A ResNet50 classification model with a single fully-connected layer in the classification head has $N_{sup}=25.56M$ trainable parameters.
%     \item Relative Location model with a ResNet50 backbone has $N_{RL}=40.30M$ trainable parameters.
%     \item ODC model with a ResNet50 backbone has $N_{ODC}=24.71M$ trainable parameters
%     \item MoCo v2 model with a ResNet50 backbone has $N_{MoCo}=27.97M$ trainable parameters.
% \end{itemize}

% \todo[inline]{pcl: I am completely lost now with this section. The previous version I saw was ok, just needed some refinement, IMO. Now everything seems different}

% We denote time complexity of running backpropagation on a model for $m$ iterations as $T(m \times n)$, where $n$ is the number of trainable parameters.
% \todo[inline]{pcl: time complexity is not a good name for this. The parallelization in GPUs precisely does not transfer the computational complexity to processing time!!}
% \todo[inline]{pcl: moreover, given this parallelization i dont think is fair to measure complexity in therms of model parameters}

% Assuming that the models are trained for the same number of epochs either on ImageNet or on ISIC-2019, we conclude that the number of iterations $m$ required to train a model corresponds to the size of the training dataset. We denote the number of iterations needed to train a model on ImageNet as $M_{ImageNet}=1.2M$ and on ISIC-2019 as $M_{ISIC}=0.02M$. Hence, time complexity of training a supervised classifier on ImageNet is $T_{sup}(M_{ImageNet}\cdot N_{sup})$,
% Relative Location on ISIC-2019 is $T_{RL}(M_{ISIC}\cdot N_{RL})$,
% ODC on ISIC-2019 is $T_{ODC}(M_{ISIC}\cdot N_{ODC})$,
% MoCo v2 on ISIC-2019 is $T_{MoCo}(M_{ISIC}\cdot N_{MoCo})$.


% Given the above notation we establish the time complexity of supervised pretraining on ImageNet as $T_{sup} = 30.67M$. In general case, training a curriculum of SSL models has time complexity of $T_{curriculum}=T_{1} + \sum^{N}_{n=2} T_{n}$. In our case, we first train individual SSL models to establish curriculum: $T_{RL} + T_{MoCo} + T_{ODC} = 0.81M + 0.56 + 0.50 = 1.87M$, and then train Relative Location and MoCo models once more (following the curriculum): $T_{RL} + T_{MoCo} = 0.81M + 0.56= 1.37M$. This gives us the total complexity of our SSL pretraining approach: $T_{total} = 1.87M + 1.37M = 3.24M$. 

% Therefore, time complexity of our approach $T_{total}$ is almost 10 times lower than time complexity of supervised ImageNet pretraining $T_{sup}$. This is especially important for novel architectures that have not yet been pretrained on ImageNet, such as the architectures tailored designed or automatically learned via Neural Architecture Search \cite{elsken2019neural} to target a specific problem.

The number of iterations required to complete the training is expressed as:

\begin{equation}
    \mathcal{I} = N \cdot E / B,
\end{equation}
where $N$ is the number of training instances, $E$ is the number of training epochs and $B$ is the batch size. Therefore, for equal batch sizes, Relative Location requires $\mathcal{I}_{RL} = 7125$ iterations to train on 20264 instances (80\% of ISIC-2019), $\mathcal{I}_{ODC} = 15832$ iterations and $\mathcal{I}_{MoCo\_v2} = 15832$ iterations. On the other hand, supervised pretraining on ImageNet with the same batch size takes $\mathcal{I}_{ImageNet} = 421875$ iterations. Finally, transferring from an SSL model to the skin-lesion recognition task requires $\mathcal{I}_{transfer} = 7125$ iterations.

Pretraining a model on a sequence of curriculum ordered pretext tasks requires to: 
\begin{enumerate}
    \item Train all $k$ individual pretext tasks and perform single-source transfer learning from them to establish the curriculum.
    \item Train $k-1$ pretext tasks in the curriculum (the first one was already trained from scratch at the step one).
\end{enumerate}

Hence, the number of required iterations required:

% \begin{equation} \label{eq:2}
%     \mathcal{I}_{curriculum} = \mathcal{I}_{task\_1} + \mathcal{I}_{task\_1}^{transfer} +  \sum^{K}_{k=2} (\mathcal{I}_{task\_k} + \mathcal{I}_{task\_k}^{transfer})
% \end{equation} 

% Because transferring to the target task takes the same number of iterations for all pretraining setups, Equation \ref{eq:2} can be rewritten as:

\begin{equation} \label{eq_final}
    \mathcal{I}_{curriculum} = \mathcal{I}_{task_1} + 2\cdot\sum^{K}_{k=2} \mathcal{I}_{task_k} + K \cdot(\mathcal{I}_{transfer})
\end{equation} \label{eq_complexity}

In our case, $k=3$ (full curriculum). Thus, $\mathcal{I}_{curriculum} = \mathcal{I}_{ODC} + 2\cdot\mathcal{I}_{RL} + 2\cdot\mathcal{I}_{MoCo\_v2} + 3\cdot{\mathcal{I}_{transfer} = 83121}$, at most.

Therefore, the complexity of our full-curriculum approach $\mathcal{I}_{curriculum}$ is almost five times lower than time complexity of supervised ImageNet pretraining $I_{ImageNet} = 421875$. 
% \todo[inline]{pcl: definition of Tsup is too far away for an easy comparison. I think is better togive all numbers for the SSL case. Then, the imagenet numbers, and you have both closer to see the difference}

This complexity reduction is especially important for novel architectures that have not yet been pretrained on ImageNet, such as architectures that are tailor-designed, or automatically learned via Neural Architecture Search \cite{elsken2019neural}, to target a specific problem.

% which in our example increases the total number of iterations to 76500 \textemdash almost 5.5 times less than supervised ImageNet pretraining.

% \todo[inline]{pcl: I would turn the ordering around. First consider the general case of N pretext tasks and, then particularize for our 3-task case. }

% \todo[inline]{pcl: Also, why not include the number of itereations in table 2? so we can refer to these numbers? Here, I also suggest to include ImageNet parameters in previous comments. kis: I included them in the text, is this fine?}

% \todo[inline]{pcl: finish with a conclusion on how our apporach is much less expensive than ImageNet, focusing on novel architectures, or architectures developed ad-hoc for a problem}

==> arXiv - SSL pretext task ordering for improved skin lesion recognition/intro.tex <==
\section{Introduction}
\label{sec:introduction}


% \todo[inline]{pcl: wher should an ack to the project go in this template? remember to ask us for a text on this
% \\ kis: in the footnote on this page I think}
% \todo[inline]{pcl: Other options for the title that I like better: 

% Improved skin lesion recognition by a multi-stage Self-Supervised Deep Learning approach

% Improved skin lesion recognition by a multi-task Self-Supervised Deep Learning approach

% Multi-stage Self-Supervised scheme for improved skin lesion recognition 

% Multi-stage Self-Supervised scheme for improved skin lesion recognition using a Deep Learning architecture

% Multi-stage Self-Supervised Deep Learning for improved skin lesion recognition

% Just some ideas, give your thoughts

% kis: I like "Improved skin lesion recognition by multi-task Self-Supervised Deep Learning"
% }

According to the American Institute for Cancer Research, skin cancer is one of the most commonly occurring cancers in humans, and affects more than one million people worldwide every year \cite{bib_cancer_report}. Timely cancer diagnosis significantly increases the patient's chances of successful recovery. Therefore, it is of paramount importance to recognize the developing cancer in its early stages. However, many malignant skin lesions might go unnoticed if primary care clinicians do not recognize them as such, due to their lack of expertise or limited diagnosis time. Recent developments in AI-based automated assessment tools led to the creation of systems with significant potential for aiding medical analysis, as acknowledged by the latest EU legislative acts \cite{bib_coordinated_plan}. In particular, AI-based systems can improve skin lesion diagnostics by signaling if qualified medical personnel is necessary for diagnosis. In this regard, methods based on dermatoscopic image analysis, that do not require biopsying the lesion, are the preferred choice for early signaling.

% For this reason automated visual assessment tools are gaining attention from the computer vision research community, as they are able to aid skin lesion diagnostics and signal if the involvement of the qualified medical doctor is necessary.
% \todo[inline]{pcl: In the previous paragraph I miss some sentence how CV can help in the process. better identification? massive analysis? patient auto-analysis? ...}
 \begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.15\textwidth}
       \includegraphics[width=\textwidth]{figures/relative location, moco, odc/201_gt.jpg}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.15\textwidth}
       \includegraphics[width=\textwidth]{figures/relative location, moco, odc/201_moco_rl_odc.jpg}
  \end{subfigure} 
  ~
  \begin{subfigure}[t]{0.15\textwidth}
       \includegraphics[width=\textwidth]{figures/relative location, moco, odc/201_odc_rl_moco.jpg}
  \end{subfigure} 
  \par\bigskip
  \begin{subfigure}[t]{0.15\textwidth}
       \includegraphics[width=\textwidth]{figures/relative location, moco, odc/0_gt.jpg}
       \caption{Original}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.15\textwidth}
       \includegraphics[width=\textwidth]{figures/relative location, moco, odc/0_moco_rl_odc.jpg}
    %   \caption{MoCo v2 $\,\to\,$ ODC $\,\to\,$ Relative location (anti-curriculum)}
    \caption{Anti-curriculum}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.15\textwidth}
       \includegraphics[width=\textwidth]{figures/relative location, moco, odc/0_odc_rl_moco.jpg}
    %   \caption{Relative location $\,\to\,$ ODC $\,\to\,$ MoCo v2 (curriculum)}
       \caption{Curriculum}
  \end{subfigure}
  \caption{Class activation maps (the brighter the more relevant the corresponding region in the image is for the model prediction) of classifiers pre-trained with pretext tasks ordered in an advantageous (curriculum) and disadvantageous (anti-curriculum) fashion. Each row corresponds to a different sample image. 
%   \todo[inline]{pcl: the figure has to be referenced in the text. Depends on the space but if we have it, I would add the samples in Figure 1 also in the corresponding section, and be more high-level (divulgative) in the caption here }
}
  \label{fig_triplets}
\end{figure}
% \todo[inline]{pcl: I would drop here the +- interval for the accuracy, and even the details that it is the balanced accuracy (not necessary for the intro). Instead add more explanation about what the do you refer with the multi-class classification problem}
As of today, leading approaches for image-based skin lesion assessment \cite{bib_isic19_winner} are based on Convolutional Neural Networks (CNNs), achieving up to 72.5\% of accuracy on the multi-class classification problem of the popular benchmark dataset\textemdash ISIC-2019 \cite{bib_ham10000, isic_part_2, bib_bcn20000}, in which skin lesions are to be classified among 8 categories (i.e., melanoma, melanocytic nevus, vascular lesion, etc.). Traditionally, these solutions are trained in a supervised learning setting where the weights of the network are initialized randomly and automatically optimized to correctly predict the labels of the data in the training set by minimizing the value of the loss function that measures correctness of model's predictions \cite{bib_sgd}.
% \todo[inline]{pcl: I think that the explanation of the loss function is too for a paper. Cn be understood as known}
% \todo[inline]{pcl: add why the dataset needs these characteristics, especially size and diversity}
This strategy poses three restrictions on the training dataset\textemdash it must be labeled, large in size and diverse \cite{bib_impact_of_size}, so that the features learned from the training data can accurately approximate those found in the validation set. For its application to dermatoscopic imaging analysis\textemdash and generally medical imaging, these conditions entail a significant obstacle, as the availability of images themselves is limited due to the privacy restrictions and rareness of certain medical conditions. Moreover, even if the data is available, annotating it requires the skills and expertise of qualified doctors, which further contributes to the difficulty of dataset creation. For these reasons, some of the largest available medical imaging datasets consist of just around 100 000 labeled images (NIH Chest X-Ray dataset \cite{bib_nih}), while most others (PAD-UFES-20 \cite{bib_pad}, TCGA-LUAD \cite{bib_ct}, Lumbar Spine MRI \cite{bib_mri}, etc.) are significantly smaller, sometimes containing only a few hundred images per dataset\textemdash tens to hundreds times less than ImageNet \cite{bib_imagenet}. This makes supervised CNN training on such data largely ineffective.
% \todo[inline]{pcl: It is a bit strange that you first particularize in dermatologists for labeling, and then talk about other type medical datasets. I would generalize to doctors/phisician (the most adequate term) in the labeling part }

% \todo[inline]{pcl: Add the reference to ImageNet here, first time mentioned}

To address the lack of data, it is beneficial to \textit{pretrain} CNN models on (preferably) domain-similar datasets to obtain a better starting point for training on the \textit{downstream task} (i.e., the target task, such as skin lesion classification) \cite{bib_how_transferable_feats}. Usually, such starting points are obtained by supervised training of a CNN model on a large and widely accepted as representative dataset, such as ImageNet~\cite{bib_imagenet}. Importantly, even when the domains of datasets used for pretraining and downstream task training differ significantly, pretraining still yields better performance than using randomly initialized weights~\cite{bib_how_transferable_feats}. Nonetheless, this limits the model selection to architectures with publicly available ImageNet-pretrained models, implying a computationally expensive and time consuming training procedure for new model architectures, or architectures designed ad-hoc for specific tasks, such as skin lesion recognition.

% \todo[inline]{pcl: I would extend last sentence a bit, something like ... new model architectures, or architectures designed ad-hoc for specific tasks such as skin lesion recognition.

%  new generalistic models can be expected to be trained in imagenet, so one can argue that is not necessary,  but not the ad-hoc ones.  
% }

% \todo[inline]{pcl: the last sentence feels disconnected with the discourse. Better change the ordering to first talk about the advantages of pretraing, and then the computational cost}
% \todo[inline]{pcl: as we discussed, this point needs to be specified, because the imediate thought is, models trained in imagenet already exist, so there is no computational cost. We can talk about the design of new architectures, maybe specifically designed for the problem}
% \todo[inline]{pcl: Previous paragraph: To better focus it, I would add an idea of the problems of obtaining labeled datasets in the medical imaging domain, and here in particular. An idea of the number and size of existing datasets. Also wotrh explaining the possible challenges: indentify malignant-non malignant (or the common names for this) and the multi-class classification. Also, probably here is a good point to include a reference to the SOTA work in the multi-class problem with accuracy numbers (that we can say in the last part of the introduction that we improve in X\% )}

In such situations, a common method to pretrain a CNN model is to use Self-Supervised Learning (SSL)\textemdash a subset of unsupervised learning methods that leverages automatically generated labels as training objectives. The SSL-driving tasks, known as \textit{pretext tasks}, vary in their formulation and aim at solving problems that do not require manually annotated data: e.g., predicting randomly applied rotations \cite{bib_rotation}, colorization \cite{bib_colorization} or solving jigsaw puzzles \cite{bib_jigsaw}. Previous works show the advantages of SSL-pretraining applied for object recognition \cite{bib_moco_v1}, where SSL-pretrained models outperform models pretrained on ImageNet in a supervised regime, and skin lesion assessment \cite{bib_ssl_robustness}, where SSL-pretraining makes models more robust to noise.

% \todo[inline]{pcl: I miss something else about these advantages. Are they in terms of performance improve? close to sota results without the labeling effort?? ... }

% \todo[inline]{pcl: if there are numbers of SSl approches to ISIC-19, i think is worth including them in the results tables.} However, to our knowledge, none of the existing state-of-the-art methods explore the effects of different orderings of pretext tasks for skin lesion recognition.

% \todo[inline]{pcl: Previous paragraph: We need to explain the potential of SSL in the skin-lesion imaging domain, alleviate the problem of unlabelled data, etc.}


% \todo[inline]{pcl: I miss in the introduction a larger summary of our work, including for example, the discussion on how we show that, curriculum ordering focus in the relevant parts of lesion image, etc.}

In this study we take a step further for SSL pretraining by showing that the consecutive use of properly ordered pretext tasks significantly improves the results on ISIC-2019, with respect to pretraining using individual pretext tasks. Curriculum learning strategies \cite{bib_curriculum_learning}  propose to order samples during training according to their learning outcomes. Inspired by these techniques, we propose orderings of pretext tasks. Specifically, we hypothesize that, given a downstream task, an advantageous ordering of pretext tasks can be obtained by sorting the tasks according to the increasing order of their individual performances. We call orderings following this rule curriculum ones. Experimental results demonstrate that curriculum orderings tend to achieve higher performance on the downstream task than the rest of the possible orderings of the explored pretext tasks.
% \todo[inline]{pcl: with respect to what? }

% \todo[inline]{pcl: we need to add here the concept of curriculum in the tasks, that is mentioned in the title. You can say something like ... different orderings explored, with better performance for those orders that follow a pretext task curriculum, inspired by curriculum learning (samples)}

% In addition to the analysis of accuracy results, we provide visual evidence that such orderings result in the models that more precisely focus on the skin lesion during inference (see an example in Figure~\ref{fig_triplets}).

In addition to the analysis of their accuracies, we provide visual evidence that automatically obtained curriculum orderings of pretext tasks results in more effective internal representations that better focus on the skin lesion (see an example in Figure~\ref{fig_triplets}), which explain the increase in classification accuracy.

% \todo[inline]{pcl: to avoid references of fig/table nombers that jump to the next line, use the symbol that I used above to create a space that cannot be separated into different lines}

% \todo[inline]{pcl: try to link these two things (accuracy and focus): an adequate ordering of pretext tasks results in effective internal representations, with a better focus on the skin lesion, which contributes in an accuracy improvement (or similar text)}

Overall, our analysis results in the following contributions:
% \todo[inline]{pcl: restrict these conclusions to the ISIC-19 problem. We cannot have more general conclusions}

\begin{itemize}
    \item We show that if pretext tasks are applied sequentially, their ordering has a significant effect on the model's accuracy after fine-tuning.
    % \todo[inline]{pcl: specify. I wouldnt talk about downstream task in general, but skin-lesion recognition}
    \item Results indicate that curriculum orderings of the evaluated pretext tasks benefit the transferred performance over models not following these orderings.
    % \todo[inline]{pcl: orderings based on indiviual accuracies does not indicate how it iis done. Specify:  ordered by increasing accuracy or other alternative way to put it }
    \item We demonstrate that\textemdash given a common architecture and using curriculum orderings, sequential SSL pretraining on ISIC-2019 dataset can outperform both supervised pretraining on ImageNet and the current winner of the ISIC-2019 challenge \cite{bib_isic19_winner}, reaching 75.44\% of balanced accuracy after fine-tuning for classification, while requiring significantly less time and resources for training.
    % \todo[inline]{pcl: Add also here that is superior to [3]}
    % \todo[inline]{pcl: if ours is the highest accuracy reported in the literature indicate it here}
\end{itemize}

% \todo[inline]{pcl: overall I find the introduction a bit imbalanced yet. With only a few text dedicated to explain the main points of the  content, advantages and findings of the work presented here.}
    


% \todo[inline]{pcl: in the contribution of accuracy performance, add the numbers}

==> arXiv - SSL pretext task ordering for improved skin lesion recognition/method.tex <==
\section{Proposed approach}
\label{sec:Methodology}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/SSL_ordering_v2.pdf}
    \caption{Proposed pretraining scheme.}
    \label{fig_ssl_ordering}
\end{figure}

\begin{table}
\centering
\caption{Accuracies for the evaluated single- and multi-source transfer settings for the ISIC-19 skin lession recognition task. The right-most column indicates whether the pretraining strategy led to a higher classification accuracy than supervised pretraining on ImageNet. The column "$\delta$" indicates how the performance of a combination of pretext tasks differs from an individual pretext task. The left-most column shows whether a combination follows Curriculum (C), Anti-Curriculum (AC) or Mixed Curriculum (MC) ordering.
% \todo[inline]{pcl: Reference in the challenge winner. C,AC;MC are not defined. Change column is not clarified. The text in the bottom could go in the caption directly}
}
\setlength{\tabcolsep}{2pt}
\label{table_combinations_no_kd}
\begin{tabular}{@{}rcccccc@{}}
\toprule
\multicolumn{1}{c}{} &
  1st task &
  2nd task &
  3rd task &
  \begin{tabular}[c]{@{}c@{}}Balanced \\ accuracy\\ (\%)\end{tabular} &
  $\delta$ (\%) &
  \begin{tabular}[c]{@{}c@{}}Better\\ than\\ ImageNet\end{tabular} \\ \midrule
-                    & Rel. loc.   &             &             & 69.52 & -     & No           \\
(AC)                 & Rel. loc.   & ODC         &             & 70.68 & 1.16  & No           \\
(MC)                 & Rel. loc.   & ODC         & MoCo v2     & 75.00 & 5.49  & \textbf{Yes} \\
(C)                  & Rel. loc.   & MoCo v2     &             & 74.10 & 4.58  & \textbf{Yes} \\
(MC)                 & Rel. loc.   & MoCo v2     & ODC         & 74.38 & 4.86  & \textbf{Yes} \\ \midrule
-                    & MoCo v2     &             &             & 72.74 & -     & No           \\
(AC)                 & MoCo v2     & ODC         &             & 72.72 & -0.02 & No           \\
(MC)                 & MoCo v2     & ODC         & Rel. loc.   & 67.00 & -5.74 & No           \\
(AC)                 & MoCo v2     & Rel. loc.   &             & 66.72 & -6.02 & No           \\
(AC)                 & MoCo v2     & Rel. loc.   & ODC         & 69.80 & -2.95 & No           \\ \midrule
-                    & ODC         &             &             & 63.52 & -     & No           \\
(C)                  & ODC         & Rel. loc.   &             & 68.23 & 4.71  & No           \\
(C)                  & ODC         & Rel. loc.   & MoCo v2     & 73.36 & 9.84  & No           \\
(C)                  & ODC         & MoCo v2     &             & 75.44 & 11.92 & \textbf{Yes} \\
(MC)                 & ODC         & MoCo v2     & Rel. loc.   & 65.73 & 2.21  & No           \\ \midrule
\multicolumn{1}{c}{} &
  \multicolumn{3}{c}{ISIC-2019 challenge winner \cite{bib_isic19_winner}} &
  72.5 $\pm$ 1.7 &
  - &
  - \\
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Supervised ImageNet} & 73.76 & -     & -            \\
\multicolumn{1}{c}{} & \multicolumn{3}{c}{No pretraining}      & 49.27 & -     & -            \\ \bottomrule
\multicolumn{7}{p{251pt}}{}\\
\end{tabular}
\end{table}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figures/SSL ordering_v2.pdf}
%     \caption{Proposed pretraining scheme.}
%     \label{fig_ssl_ordering}
% \end{figure*}

% \todo[inline]{pcl: In the explanation of the approach indicate both advantages: computational cost, and performance over imagenet pretraining}

% \todo[inline]{pcl: When indicating the sequential ordering, you can keep how to order them as an open question to explore, (the generation of an efficient curriculum), which is explored in the paper.  Then you can mention that the results show ordering by individual pretext task accuracy results in the best option.}

% \todo[inline]{pcl: focus more from the beginning on skin, and that the target is to benefit from this SSL pretraining to improve the accuracy}

% \todo[inline]{pcl: you use a bunch of terms for SSL that may be confusing, architecture, models, task. Try to unify}

In this study we propose to increase the accuracy on the ISIC-2019 multi-class problem by improving the pretraining pipeline, frequently applied in transfer learning approaches to the skin lesion recognition problem. The basic idea of our method (see Figure \ref{fig_ssl_ordering}) is to extend the recent works on SSL pretraining for skin lesion recognition and
leverage multiple, instead of a single, pretext tasks in the pretraining stage. 

\subsection{Preliminaries}

To clarify the proposed approach we first formalize the notation used in this work, following the nomenclature proposed in previous works \cite{bib_survey_tl}:

% \todo[inline]{kis: help me add blank lines between the definitions}
% \todo[inline]{pcl: check the vspaces below. I dont know if this is correct with the journal format, but they will anyway reformat everything at the end, usually f***ing all the format you like. You will see ...}

\vspace{0.2cm}

\textit{Domain}: A domain $\mathcal{D} = \{\mathcal{X}, P(X)\}$ is comprised of the complete feature space $\mathcal{X}$ (i.e., all images) and a marginal distribution $P(X)$, where $X=\{x|x_i \in \mathcal{X}, i=1,..., n\}$ is the set of images defining the domain (i.e., skin lesion images).

\vspace{0.2cm}

\textit{Task}: A task $\mathcal{T}=\{\mathcal{Y}, \mathcal{F}\}$ is comprised of the label space $\mathcal{Y}$ (i.e., melanoma, melanocytic nevus,...) and the implicit decision function $\mathcal{F}$ which is expected to be learned by the model from the input data (i.e., conditional probability of labels, given the samples).

\vspace{0.2cm}

\textit{Transfer learning}: Given (a) data distribution(s)  $\{\mathcal{D}_{S}, \mathcal{T}_{S_i}|i=1,..., m\}$ drawn from the \textit{source} ($S$) domain(s) and task(s), and a data distribution $\{\mathcal{D}_{T}, \mathcal{T}_{T}\}$ drawn from the \textit{target} ($T$) domain and task, transfer learning uses the knowledge from the source domain(s) to improve the performance of the decision function $\mathcal{F_T}$ on the target domain.
% \todo[inline]{pcl: do we need to consider multiple target domains? the definition of {DT,TT} does, but not the last part, or the following definitions. To simplify, I would use a single target domain.}

\vspace{0.2cm}

\textit{Single-source transfer learning}: Transfer learning setup in which $m=1$. In other words, the knowledge is transferred from a single source domain to the target domain. Most transfer learning approaches follow single-source scenario.

\vspace{0.2cm}

\textit{Multi-source transfer learning}: Transfer learning setup in which $m \ge 2$. In other words, the knowledge is transferred from multiple source domains to the target domain.

\vspace{0.2cm}

% \todo[inline]{pcl: it is not really the general case, as the general case could use different domains in each step. To simplify the description of the process, I would define both restrictions at the same time. Single source domain, equal to the target domain. Before that you can add a sentence saying that the general multi-source transfer learning could contemplate different source domains}
\subsection{Self-supervised Curricula}
With these definitions, we formulate the proposed approach as follows: given a single source domain and $k$ source tasks $\{\mathcal{D}, \mathcal{T}_{S_i}|i=1,..., k\}$, we define a multi-source transfer learning approach that uses the knowledge from $\{\mathcal{D}, \mathcal{T}_{S_i}\}$ to improve the performance of the learned target decision function $\mathcal{F}_T$. In this setting, the knowledge is sequentially transferred from $\{\mathcal{D}, \mathcal{T}_{S_{i}}\}$ to $\{\mathcal{D}, \mathcal{T}_{S_{i+1}}\}$ (the first task $\mathcal{T}_1$ is trained from scratch). At step $k$ we transfer the knowledge from $\{\mathcal{D}, \mathcal{T}_{S_k}\}$ to the target task $\{\mathcal{D}, \mathcal{T}_T\}$.


% To split the problem further, we consider that the first task $\mathcal{T}_{S_1}$ is already trained on the source domain $\mathcal{D}_S$, and define $k-1$ single-source transfer learning problems, where the $i$-th problem transfers the knowledge from $\{\mathcal{D}_{S}, \mathcal{T}_{S_{i}}\}$ to improve the performance of the decision function $\mathcal{F}_{S_{i+1}}$ of the task $\mathcal{T}_{S_{i+1}}$ on the source domain $\mathcal{D}_S$ for $i=1,.., k-1$. 

% \todo[inline]{pcl: The last sentence is quite confusing. Since in our problem, the source domain and target domain are the same, why not stating that upfront and then define all steps in a unified way?

% kis: I think in this paragraph we should keep it more general: source and target domains are different. But in the next one, yes, it can make it clearer. Marcos?

% mev: well, the thing is that here you are saying that this is the proposed approach...maybe it should be clarified at the end at least, indicating that for SSL learning the source and the target domains are the same. 

% This can be done using the next paragraph, instead of starting with In other words, start with Notice, that, as in SSL the source ($\mathcal{D}_{S}$) and target ($\mathcal{D}_{T}$) domains are the same, the whole process can be formalized as the training of $i, i=1,...,k$ pretext tasks ...

% }

Note, that in our case the source $\mathcal{D}_S$ and the target $\mathcal{D}_T$ domains are the same, therefore, the whole process can be viewed as the sequential training of $k+1$ models on the source domain.


% \todo[inline]{pcl: shouldnt it be just ... train k-1 pretext tasks ... ? The k-th training is the targest task, isnt it? 

% kis: no, you have $k$ pretext tasks, so you have $k-1$ transfers between them and the $k_{th}$ one refers to transferring from the last pretext task to the target task (the first step is training the first task from scratch, but it's not transfer learning, it's just normal training). 

% mev: maybe the noise comes from the first part when you say that  To split the problem further, we consider that the first task $\mathcal{T}_{S_1}$ is already trained on the source domain $\mathcal{D}_S$, and define $k-1$ single-source transfer learning problems, where the $i$-th problem transfers the knowledge ...  , is this really needed? Could it be simplified?

% } 

% \todo[inline]{mev: I change j for i, why did you use j here?}

% The first pretext task $\mathcal{T}_{S_1}$ starts the training from the random starting point with random weights, thereby, not relying on transfer learning. $\mathcal{T}_{S_1}$ uses the data from the source domain $\mathcal{D}_S$ and the automatically generated labels from its label space $Y_{S_1}$. Then, for $i=1,..., k-1$ each next pretext task $\mathcal{T}_{S_{i+1}}$ begins training from the point at which the previous one stopped by copying the backbone network weights (i.e., copying the learned decision function), and using its own label space $\mathcal{Y}_{S_{i+1}}$. Finally, the target decision function $\mathcal{F}_T$ is learned using the target label space $\mathcal{Y}_T$, representing the actual labels in a training set of ISIC-2019 images.

% \todo[inline]{pcl: this can also be simplified. You dont need to differenciate how you copy weights in the pretext tasks and target task, because the processs is the same. Define it in a unified way, and mention ,after, that for the first task you start from random weights.

% kis: I'm confused with this already, I'll get back to it tomorrow
% }


% In particular, we suggest using a combination of SSL models in the pretraining stage instead of relying on costly supervised pretraining on ImageNet. As illustrated in Figure \ref{fig_ssl_ordering}, we sequentially train a series of pretext tasks on the unlabeled data of the target dataset. Finally, we initialize the weights of the classification model by copying the weights learned by the backbone of the last pretext task, and begin training on the downstream task in a supervised manner. 
% \todo[inline]{pcl: probably is worth to clarify that the weights obtained after a SSL training stage are transfered to the as initial weights for the next}

% \todo[inline]{pcl: i think this next may better go in next section. You give here the general method, and in Section 4 you can mention that in our setup, k=3, to have the different categories, the discussion on how it is expected that 1 task per category is enough, and our selection of tasks. Here, you can keep that it is an open question how to order the k pretext taks, and, that it will be shown in Section IV that the order of pretext tasks}

Currently, optimal ordering of $k$ pretext tasks remains an open question. We define the best performing ordering as the curriculum one and make a hypothesis that it coincides with the ordering $\mathcal{A}_{1}, \mathcal{A}_{2},... \mathcal{A}_{k}$ of accuracies obtained with each pretext task individually, where $\mathcal{A}_{1} \leq \mathcal{A}_{2} \leq ... \leq \mathcal{A}_{k}$. Further, in Section \ref{sec:Experiments}, we present experimental findings that support this hypothesis.
% It will be shown in Section \ref{sec:Experiments} that it has crucial effect on the accuracy of skin-lesion recognition after transfer learning. 

% \todo[inline]{pcl: i think there is a problem on how you use decision function here, given the way you have defined it. it does not only refer to the embeddings, but the whole model, and they are different on each step, the last part for sure ... }

% \todo[inline]{pcl: in the introduction you mention a work that uses parallel pretext task training on the skin-image domain. How do we relate to this work= i.e. do we have a way to justify the use of sequential training only?}

==> arXiv - SSL pretext task ordering for improved skin lesion recognition/related_work.tex <==
\section{Related work} \label{Sec:related}

This section presents a brief overview of the current state-of-the-art in skin lesion recognition and discusses the use of Self-Supervised and Supervised Learning and in the presence of limited training data, specifically, medical imaging data.

\subsection{Limitation of traditional approaches to image recognition}

Most image recognition approaches are based on CNNs. A common strategy to improve a CNN's prediction accuracy on a given task is to increase the complexity of the model. This is done either by significantly changing the underlying network's architecture (i.e., AlexNet \cite{bib_alexnet} vs. VGG \cite{bib_vgg} vs. ResNet \cite{bib_resnet}) or adjusting its depth \cite{bib_resnet} and/or width \cite{bib_wide_net}. However, despite the growing performance on the ImageNet challenge, such approaches do not address the large limitation of any CNN, that is especially relevant to medical imaging datasets: their poor ability to generalize and learn efficient representations with limited training data.

Alternatively to changing the models themselves, one might resort to using ensembles of various networks or the same network trained multiple times (trials) with different initializations \cite{bib_ensembles_in_ml, bib_ensembles_nature}. However, this approach is very computationally expensive (as it requires to train the multiple models that comprise an ensemble, and later collect each model's prediction during inference). Furthermore, this paradigm is also not trivial to adapt to new tasks/domains, as it may imply the adaption of every model in the ensemble. 

\subsection{Current state of skin lesion recognition}

Due to privacy restrictions, to the relatively low rate at which certain medical conditions develop, and to the uneven distribution of suitable capture devices worldwide, a very small amount of medical imaging data is publicly available. In the subfield of skin lesion analysis, one of the largest accessible collections of imaging data is the International Skin Imaging Collaboration (ISIC) dataset that aggregates the data from other sources, such as HAM\_10000 dataset \cite{bib_ham10000}, MSK dataset \cite{isic_part_2} and BCN\_20000 dataset \cite{bib_bcn20000}. Annual public challenges based on the ISIC dataset target multi-class (predicting the exact type of a skin lesion) or binary (malignant vs. benign) classification problems. Whereas the latter can be considered an almost solved problem (ISIC-2020\textemdash a binary melanoma recognition problem\textemdash challenge winners achieved 0.949 on ROC AUC metric), the multi-class problem proposed in ISIC-2019 is still an open one, where the best reported approach \cite{bib_isic19_winner} currently reaches only 72.5\% $\pm$ 1.7\% of \textit{balanced accuracy} (average per-class accuracy).

Although ISIC-2019 is the largest publicly available skin lesion dataset with multi-class annotations, containing over 25000 labeled images, its size is small compared with those used for standard CNN training in well established tasks. Moreover, the number of samples per class ranges from 239 to 12875, making it highly imbalanced and further complicating CNN training\textemdash e.g., a vanilla ResNet-50 \cite{bib_resnet} does not reach 50\% of balanced accuracy, as shown in Table \ref{table_combinations_no_kd}. Some works address this issue by designing new loss functions that account for severe class imbalances \cite{bib_isic_loss_functions}. However, the general trend seems to be increasing the complexity of neural models and utilizing deeper architectures, such as DenseNets \cite{bib_densenet} or very deep ResNets \cite{bib_resnet}. Continuing in the same direction, the top three best performing approaches in ISIC-2019 skin lesion diagnosis challenge are based on ensembles of neural networks that leverage multiple models to infer predictions  \cite{bib_isic19_winner, bib_isic_19_winner_2, bib_isic_19_winner_3}. 
% \todo[inline]{pcl: i still feel that the description of the approaches to skin-lesion recognition are too scarce. You only mention 3 worrks, which all do ensemble learning. What about others? arent there any? Any non-DL algorithm worth mentioning?}


% \todo[inline]{pcl: i dont understand the puropse of this sections B and C here, when you have already talked about the way that ensembling is used in skin-lesion to imporve the performance. In my view, this texts, (or parts of them) should be integrated in the section above. maybe following these ideas: accuracy has been improved generally by increasing model complexity, however, this doesnt work for limited data as skin (resnet example). This can be improved by ensembling,and references to the sota papers. I do not know if this structure comes from a suggestion from Marcos, and maybe is worth discussing it before doing the changes}


\subsection{Transfer learning and Self-Supervised Learning}

% \todo[inline]{pcl: i would use the complete name (SSL in the title)}

A different and popular approach to increase the classification accuracy of deep learning architectures is transfer learning: using a model trained for one task as a starting point for training for a different task. Recent studies introduce strategies for pretraining models without relying on labelled data \cite{bib_rotation, bib_moco_v1}. This is achieved by using SSL-based methods that solve a \textit{pretext task} by formulating objectives that do not require manually labelled data. It is assumed that solving pretext tasks requires a high-level understanding of the data and, therefore, allows to learn efficient visual representations. Hereby, the features learned through solving \textit{pretext tasks} are considered to be starting points suitable for transfer learning. For instance, a well-known \textit{pretext task}\textemdash rotation prediction~\cite{bib_rotation}\textemdash generates training labels that encode a series of rotations applied to the input image, anticipating that the information required to correctly rotate an image requires the \textit{learning} of some fundamental object qualities.

\subsection{Curriculum learning}
% \todo[inline]{pcl: i changed the woring of the phrase above. Is there any better word for starting point? refering to transfer learning? }

% \todo[inline]{pcl: I miss a bit more on the different works that tackled the problem? References and categories of algorithms if possible. Probably you can extract this information of the related work of previous papers}

Although the number of existing SSL strategies is constantly increasing, a categorization according to the underlying label generation strategy can be used to assign them to one of three categories: \textbf{geometric} (Rotation prediction \cite{bib_rotation}, Relative patch location \cite{bib_relative_location}, Jigsaw puzzles \cite{bib_jigsaw}),  \textbf{clustering} (Deep Clustering \cite{bib_dc}, Online Deep Clustering \cite{bib_odc}, ClusterFit \cite{bib_clusterfit}) and  \textbf{contrastive} (Momentum Contrast \cite{bib_moco_v1, bib_moco_v2}, Bootstrap Your Own Latent \cite{bib_byol}, Non-Parametric Image Discrimination \cite{bib_npid}, Simple Framework for Contrastive Learning of Visual Representations \cite{bib_simclr}). 

Relative patch location prediction, being a typical \textbf{geometric} SSL model, splits an input image into patches, then samples two adjacent ones and trains to predict their relative location. On the other hand, \textbf{clustering} SSL models, such as Online Deep Clustering (ODC), use classical clustering algorithms to generate intermediate training labels. Finally, \textbf{contrastive} models rely on the use of the contrastive loss function to discriminate between positive and negative samples. Often the negative samples are generated through the data augmentations of positive samples, as it is done in the case of Momentum Contrast (MoCo) model.

Currently, regarding the accuracies achieved using ImageNet as the downstream classification task, \textbf{contrastive} models outperform \textbf{geometric} and \textbf{clustering} ones: MoCo v3 \cite{bib_moco_v3}\textemdash81.0\%, SimCLR v2\cite{bib_simclr_v2}\textemdash79.8\% and BYOL\cite{bib_byol}\textemdash79.6\%, while the closest \textbf{clustering} model\textemdash DeepCluster v2\cite{bib_dc}\textemdash yields only 75.2\% of accuracy and a classic \textbf{geometric} model\textemdash Rotation prediction\textemdash reaches 55.4\% of accuracy.

\subsection{SSL in skin lesion recognition}

The promise of learning useful representations without requiring labelled data led to the applications of SSL strategies to the medical imaging, where data labelling is challenging. In particular, a number of recent works target the skin lesion recognition problem leveraging SSL approaches for model pretraining. This narrows the gap between SSL and fully supervised pretraining on ImageNet but, in most cases, does not yet close it. For example, a recently proposed approach \cite{bib_topology} reaches 80.6\% of accuracy on a multi-class ISIC-2018 classification problem by employing self-supervision to obtain transformation-invariant features. Specifically, features extracted at each epoch from the image decoder module of a CycleGAN architecture \cite{bib_cyclegan} are assigned to $N$ clusters without a prior knowledge of $N$, using the maximum modularity clustering algorithm \cite{bib_modularity_clustering}. The memberships of the samples are used as pseudo-labels to optimize the features. A different study compares the individual performances of five existing SSL models \cite{bib_ssl_evaluation_2021} (BYOL \cite{bib_byol}, MoCo \cite{bib_moco_v2}, SimCLR \cite{bib_simclr}, InfoMin \cite{bib_infomin}, SwAV \cite{bib_swav}) on the ISIC-2019 data, but only considers the binary classification problem, reaching 0.956 on the standard for binary problems metric\textemdash ROC AUC (area under the precision-recall curve). On the contrary, another recent work does consider the multi-class skin lesion classification problem and shows that SimCLR pretraining outperforms supervised pretraining \cite{bib_super_dataset}. However, this study relies on a private dermatoscopic dataset containing over 450 000 samples. Nevertheless, there is a gap in the current state-of-the-art as, to our knowledge, none of the existing approaches considers more than one SSL task in the pretraining stage, thus, limiting the resulting performance by not taking advantage of the pretext tasks of different nature. Moreover, with seldom exceptions, most works that use SSL pretraining in the skin lesion domain rely only on \textbf{contrastive} models (as these are generally the most accurate ones), thus, the potential contributions of \textbf{clustering} and \textbf{geometric} models are still barely explored. Finally, a multi-class skin lesion recognition problem is relatively unexplored by SSL methods, as the majority of works focus on the binary melanoma recognition task, and only a few studies target the multi-class problem of the older (and smaller) versions of the ISIC dataset. 

% \todo[inline]{pcl: I miss a better organization for this part. Can we reorganize it this way? (if something I say is not true discuss it) 1. ... a numberof recent works target the skin lesion recognition problem leveraging SSL  approaches (add some general conclusion on their performance wrt supervised counterparts) 2. we say that most of the ssl skin works tackle the binary classif problem, 3. talk about the first two works you mention (here you need to say something about the performance, you say what they do but not mention if they outperform or not supervised alternatives). 4. mention that only ¿one? ssl work tackles the multi-class problem, and then your description of it.}
% \todo[inline]{pcl: When you start talking about the limitations, explicitely mention the potential of multiple SSL: better performance to single SSL, by the aggretgation of different nature tasks, not for the sake of exploring it. Also you can say that the multi-class is relatively unexplored by ssl methods, as the only work you mention uses extra data that makes comparison difficult to works that are restricted to the ISIC dataset}

% \todo[inline]{pcl: this last sentence refers to skin? or other vision task? If the latter, it should be moved to the previous paragraph}
% \todo[inline]{pcl: Here you should ellaborate more on what they do in these SSL-skin works (and what is missing) so you can argue that our work improves/completes/extends theirs}



A promising method for improving the accuracy of deep learning architectures emerges from the careful selection and ordering of training samples\textemdash curriculum learning \cite{bib_cl_starting_small, bib_shaping, bib_curriculum_learning}. The idea behind it is that, inspired by human learning processes, the training of deep learning architectures may benefit from ordering of data samples based on some evidence of their \textit{complexity}, e.g., their contribution in the training loss. 

Generally, a curriculum of samples starts by using for training those samples that are learned faster and progressively incorporates the rest. For visual tasks, reported results indicate that curriculum training results in models that yield better performance than those obtained when samples are selected at random \cite{bib_curriculum_learning}. However, despite the benefits of curriculum learning at the samples level, to our knowledge no study investigates the effects of a different orderings of models pre-trained with multiple sequential tasks. In this work we define a curriculum order of pretext tasks that optimizes the performance of a model pre-trained sequentially on those tasks. Finally, we investigate applications of curriculum ordering of pretext tasks and their effects on the skin lesion recognition performance.


% \todo[inline]{pcl: if the model level term is common, fine, but for me sounds misleading. it could give the idea we are ordering architectures }

% \todo[inline]{pcl: proposed alternative: ... investigates the effects of a curricular ordering in models pre-trained by multiple pretext tasks, i.e. a curriculum order could be defined for a set pretext tasks, which optimizes the performance of a model pre-trained sequentially for those tasks.}
% \todo[inline]{pcl: I would finish with a sentence saying that we investigate this idea and its benefits in skin}
